Do ReLU Networks Have An Edge When Approximating Compactly-Supported Functions?

We study the problem of approximating compactly-supported integrable functions while implementing their support set using feedforward neural networks. Our first main result transcribes this "structured" approximation problem into a universality problem. We do this by constructing a refinement of the usual topology on the space $L^1_{\operatorname{loc}}(\mathbb{R}^d,\mathbb{R}^D)$ of locally-integrable functions in which compactly-supported functions can only be approximated in $L^1$-norm by functions with matching discretized support. We establish the universality of ReLU feedforward networks with bilinear pooling layers in this refined topology. Consequentially, we find that ReLU feedforward networks with bilinear pooling can approximate compactly supported functions while implementing their discretized support. We derive a quantitative uniform version of our universal approximation theorem on the dense subclass of compactly-supported Lipschitz functions. This quantitative result expresses the depth, width, and the number of bilinear pooling layers required to construct this ReLU network via the target function's regularity, the metric capacity and diameter of its essential support, and the dimensions of the inputs and output spaces. Conversely, we show that polynomial regressors and analytic feedforward networks are not universal in this space.

==> Rebuttals/Rebuttals.tex <==
Dear Action Editor,

Thank you very much for taking the time to manage our submission.

We would like to clarify that our paper is ultimately about the approximation of compactly supported Lebesgue-integrable functions and how two different popular classes of deep learning models fair when approximating such functions; though we admit that there are some points in the manuscript’s presentation which can be tweaked to realign our results with our presentation of them.
Unlike for the broader class of locally Lebesgue-integrable functions where one wants to approximate the map $x\mapsto f(x)$.  When approximating essentially compactly-supported Lebesgue-integrable functions, it is natural to hope to learn more, since such functions carry more structure than locally Lebesgue-integrable functions do.  Therefore, the main objective of this manuscript is to show that ReLU networks with bi-linear pooling are better suited to the approximation of essentially compactly-supported Lebesgue integrable functions than their analytic counterparts; not that ReLU networks are better than analytic networks for the approximation of all functions (e.g. we had some comments relating the clear advantage of tanh networks to ReLU networks for physics-inspired learning the paper paper’s discussion section)

This brings us to your question:
“As far as I can tell, you have not proven that there does not exist a refinement of the same topology of locally Lebesgue-integrable functions in which networks with analytic activations are dense, but networks with piecewise linear activations are not. (That is, you’ve not ruled out such a refinement.)… Is that correct?”

“Yes” and “no”. Let us first explain the “no” part:
The topology which we construct (Theorem 1) exhibits this “separation phenomenon” when approximating compactly supported Lebesgue-integrable functions. We do so by constructing a topology which satisfies four main properties: namely, the ReLU networks with bilinear pooling are dense therein (Theorem 1 (i)), the topology refines the topology on $L^1_{\operatorname{loc}}(\mathbb{R}^d,\mathbb{R}^D)$ (Theorem 1 (ii)), and most importantly the approximation of a compactly supported function requires its approximation in $L^1$ as well as the correct identification of its support up to a well-behaved discretization of $\mathbb{R}^d$ formalized by our good a.e. partitions (Theorem 1 (iii) and (iv)). Indeed one can construct another topology on $L^1_{\operatorname{loc}}(\mathbb{R}^d,\mathbb{R}^D)$ in which the analytic networks satisfy (i) and (ii); however, in such a topology the analytic networks satisfy Theorem 1 (iii) precisely due to analyticity and the fact that the said topology refines the topology on $L^1_{\operatorname{loc}}(\mathbb{R}^d,\mathbb{R}^D)$. Therefore, our last iteration of Theorem 1 (iii) prohibits the interchangeability of the roles of these two models in the theorem’s statement.

For the “Yes” part:
After the discussion with the reviewer and yourself, we feel that there are a few places in our manuscript in which the writing can be properly aligned to the results which we demonstrate; e.g.
- instead of saying, “Our main result demonstrates that deep networks with piecewise linear activation (e.g. ReLU or PReLU) are fundamentally more expressive than deep feedforward networks with analytic (e.g. sigmoid, Swish, GeLU, or Softplus) activation functions.”
- rather, we demonstrate that “Our main result demonstrates that deep networks with piecewise linear activation (e.g. ReLU or PReLU) are better suited to the approximation of compactly supported Lebesgue-integrable functions than deep networks with analytic (e.g. sigmoid, Swish, GeLU, or Softplus) activation functions.”
We would like to revise our manuscript by implementing these short writing changes, which accurately reflects what we have shown. We feel that, with these changes, the manuscript’s results and message will be properly calibrated; whereas they were not in the earlier iterations, and we feel that this rightfully spurred the helpful discussion.

Would you also agree that these short changes are appropriate and that they solve the concerns brought up about the misalignment of the paper’s results and its message?

Best,
The Authors
